SUPER Learning: A Supervised-Unsupervised Framework for Low-Dose CT Image Reconstruction

Recent years have witnessed growing interest in machine learning-based models and techniques for low-dose X-ray CT (LDCT) imaging tasks. The methods can typically be categorized into supervised learning methods and unsupervised or model-based learning methods. Supervised learning methods have recently shown success in image restoration tasks. However, they often rely on large training sets. Model-based learning methods such as dictionary or transform learning do not require large or paired training sets and often have good generalization properties, since they learn general properties of CT image sets. Recent works have shown the promising reconstruction performance of methods such as PWLS-ULTRA that rely on clustering the underlying (reconstructed) image patches into a learned union of transforms. In this paper, we propose a new Supervised-UnsuPERvised (SUPER) reconstruction framework for LDCT image reconstruction that combines the benefits of supervised learning methods and (unsupervised) transform learning-based methods such as PWLS-ULTRA that involve highly image-adaptive clustering. The SUPER model consists of several layers, each of which includes a deep network learned in a supervised manner and an unsupervised iterative method that involves image-adaptive components. The SUPER reconstruction algorithms are learned in a greedy manner from training data. The proposed SUPER learning methods dramatically outperform both the constituent supervised learning-based networks and iterative algorithms for LDCT, and use much fewer iterations in the iterative reconstruction modules.

==> Algorithm_r2.tex <==
\section{Algorithm}\label{sec:algorithm}
The proposed SPULTRA algorithm is based on a pre-learned union of sparsifying transforms. The process of learning such a union of transforms from a dataset of image patches has been detailed in~\cite{pwls-ultra2018}. The learning problem in \cite{pwls-ultra2018} simultaneously groups the training patches into $K$ \DIFadd{classes }and learns a transform in each \DIFadd{class }along with the sparse coefficients (in the transform domain) of the patches. This learning is accomplished by an alternating algorithm (see~\cite{pwls-ultra2018}). 
This section focuses on describing the algorithm in the reconstruction stage for SPULTRA, i.e., for \eqref{eq:P0}.

%Due to the nonconvexity of the data-fidelity term caused by the SP model, we propose to design quadratic surrogate functions for this term in an iterative way. In each iteration, the cost function \ref{eq:P0} becomes a classical quadratic data-fidelity term plus a ULTRA regularizer. With the help of alternating strategy, the problem is optimized within each iteration via alternating between the image update step, that optimizes the quadratic subproblem, and the sparse coding and clustering step which have closed-form solutions \cite{wen:14:sos}. 

The data-fidelity term $\mathsf{L}(\x)$ in \eqref{eq:P0} is nonconvex when the electronic noise variance $\sigma^2$ is nonzero. It is challenging to directly optimize such a logarithmic nonconvex function. We propose to iteratively design quadratic surrogate functions for this data-fidelity term $\mathsf{L}(\x)$. In each iteration, we optimize the surrogate function that is a quadratic data-fidelity term together with the ULTRA regularizer using alternating minimization that alternates between an image update step and a sparse coding and clustering step that has closed-form solution~\cite{wen:14:sos}. We use the relaxed OS-LALM algorithm for the image update step~\cite{nien:16:rla}. We perform only one alternation between the two steps for each designed surrogate function, which saves runtime and works well in practice.

%In the following, we first illustrate the surrogate functions design for the data-fidelity term. Then, we describe the image update step, and the sparse coding and the clustering step.
\vspace{-0.1in}
\subsection{Surrogate function design} \vspace{-0.05in}
We design a series of quadratic surrogate functions for $\mathsf{L}(\x)$ as follows:
\begin{equation}\label{eq:surrogate}
\begin{aligned}
\phi(\x;\x^n) &= \mathsf{L}(\x^n) + \bm{d}_h(l^n)\A(\x - \x^n)\\
&\qquad+\frac{1}{2}(\x - \x^n)^T\A^T\W^n\A(\x - \x^n),			
\end{aligned}
\end{equation}
where $(\cdot)^n$ denotes values at the $n$th iteration and ${\bm{d}_h(l^n) \in \mathbb{R}^{N_d}}$ is a row vector capturing the gradient information and is defined as $\bm{d}_h(l^n) \triangleq [\dot{h_i}(l_i^n)]_{i = 1}^{N_d}$. The curvatures of the $n$th updated parabola (surrogate) are described by $\W^n\triangleq \text{diag}\{c_i(l^n_i)\}$. In this paper, we use the optimum curvatures \cite{TMI99} that are defined as follows:
\begin{equation} \label{eq:OptCuv}	
c_i(l^n_i) =  \begin{cases}
\big[2\frac{h_i(0) - h_i(l_i^n) + (l_i^n)\dot{h_i}(l_i^n)}{(l_i^n)^2}\big]_+, &l_i^n > 0\\
\big[\ddot{h_i}(0)\big]_+, &l_i^n = 0, 
\end{cases}
\end{equation}
where $\ddot{h}_i$ is the second-order derivative, and operator $[\cdot]_+$ sets the non-positive values to zero. In practice, we replace negative values with a small positive number so that the diagonal matrix $\W^n$ is invertible. 
Due to numerical precision, \eqref{eq:OptCuv} might become extremely large when $l_i^n$ is nonzero but small. To avoid this problem, we use an upper bound of the maximum second derivative $\big[\ddot{h_i}(0)\big]_+$ for the curvature $c_i(l^n_i)$ when $l_i^n > 0$ \cite{TMI99}.

By ignoring the terms irrelevant to $\x$ in \eqref{eq:surrogate}, we get the following equivalent form of $\phi(\x;\x^n)$:
%We can rewrite \eqref{eq:surrogate} as follows:
%\begin{equation}\label{deduce1}
%\begin{aligned}
%\phi(\x;\x^n) &= \frac{1}{2}||\tilde{y}^n - \A\x||_{\W^n}^2  +\mathsf{L}(\x^n) \\
%&- \frac{1}{2}\bm{d}_h(l^n)(\W^n)^{-\frac{1}{2}}[\bm{d}_h(l^n)(\W^n)^{-\frac{1}{2}}]^T,
%\end{aligned}
%\end{equation}	
%with $\tilde{y}^n \triangleq \A\x^n -\big(\W^n\big)^{-1}[\bm{d}_h(l^n)]^T$.
%Ignoring the terms that do not depend on $\x$ and dropping the superscript $n$ for $\W$ for notational simplicity, we get the following equivalent form of $\phi(\x;\x^n)$:
\begin{equation}\label{deduce2}
\phi(\x;\x^n) \equiv \frac{1}{2}||\tilde{\y}^n - \A\x||_{\W^n}^2,
\end{equation}	
where ``$\equiv$'' means equal to within irrelevant constants of $\x$, and $\tilde{\y}^n \triangleq \A\x^n -\big(\W^n\big)^{-1}[\bm{d}_h(l^n)]^T$. The overall surrogate function at the $n$th iteration for the penalized-likelihood objective function \DIFadd{$G(\x)$} in \eqref{eq:P0} is then
\begin{equation}\label{eq:surr_all}
\Phi(\x;\x^n) = \frac{1}{2}||\tilde{\y}^n - \A\x||_{\W^n}^2 + \R(\x),\ \DIFadd{\text{s.t.}\ \x \in \mathcal{X}.}
\end{equation}

We \DIFadd{descend} the surrogate function $\Phi(\x;\x^n)$ in \eqref{eq:surr_all} by alternating \DIFadd{once} between an image update step, and a sparse coding and clustering step.

\vspace{-0.1in}
\subsection{Image Update Step}\vspace{-0.05in}
In the image update step, we update the image $\x$ with fixed sparse codes $\{\z_j\}$ and \DIFadd{class} assignments $\{C_k\}$. The relevant part of the majorizer for this step is 
\begin{equation}\label{eq:Phi1}
 \begin{aligned}
 \Phi_1(\x;\x^n) = \phi(\x;\x^n)  + \beta \sum_{k=1}^{K} \sum_{j\in C_k} \tau_j \|\omg_k \P_j \x - \z_j\|^2_2
 \end{aligned}
 \end{equation}
\DIFadd{Although we have a box} constraint on $\x$\DIFadd{, i.e., $\x \in \mathcal{X}$, in practice, the upper bound $x_{\mathrm{max}}$ can be set high such that it will not be active. We applied the }relaxed OS-LALM algorithm~\cite{nien:16:rla} \DIFadd{to minimize }\eqref{eq:Phi1} \DIFadd{with the constraint. This algorithm is } shown in Algorithm \ref{alg: spultra-alg} (steps 7-10). The OS-LALM method uses majorizing matrices. In particular, the matrix $\A^T\W^n\A$ is majorized by \DIFadd{$\D_{\A} \triangleq \text{diag}\{\A^T\W^n \A \mathbf{1}\}$, where $\mathbf{1}$ denotes a vector of ones.} Denoting the regularization term in \eqref{eq:Phi1} as $\R_2(\x)$, its gradient is 
\begin{equation}\label{eq:grad_r2}
\nabla \R_2(\x) = 2\beta\sum_{k=1}^{K} \sum_{j\in C_k} \tau_j \P_j^T \omg_{k}^T (\omg_k \P_j \x - \z_j ).
\vspace{-0.05in}
\end{equation}
The Hessian of $\R_2(\x)$ is majorized by the following diagonal matrix:
\begin{equation}\label{eq: D_R}
%\begin{aligned}
\D_{\R} \triangleq 2\beta \bigg\{\max_k \|\omg_{k}^T\omg_{k}\|_2\bigg\}\sum_{k=1}^{K} \sum_{j\in C_k}\tau_j \P^T_j \P_j .
%\end{aligned}
\end{equation}
The (over-)relaxation parameter $\alpha \in [1,2)$ and the parameter $\rho_t >0$ decreases with iterations $t$ in OS-LALM according to the following equation \cite{nien:16:rla}:
\begin{equation}\label{eq:rho}		
\rho_t(\alpha)= \begin{cases}
1,      &  t=0\\ 
\frac{\pi}{\alpha(t+1)}\sqrt{1-\big(\frac{\pi}{2\alpha(t+1)}\big)^2},     &  \text{otherwise.}
\end{cases}
\vspace{-0.1in}
\end{equation}	
\vspace{-0.1in}
\subsection{Sparse Coding and Clustering Step}
Here, with $\x$ fixed, we jointly update the sparse codes and the \DIFadd{class }memberships of patches. The relevant part of the cost function for the sparse coding and clustering step is 
\begin{equation}\label{eq:codes-clusters} 
\min_{\{\z_j, C_k\}} \sum_{k=1}^{K}  \bigg\{  \sum_{j\in C_k} \tau_j \{\|\omg_k\P_j \x - \z_{j}\|^2_2 + \gamma_c^2\|\z_j\|_0 \}\bigg\} .
\end{equation}
\DIFadd{Problem \eqref{eq:codes-clusters} is separable in terms of the patches, so each patch is clustered and sparse coded independently in parallel. The optimal sparse code $\z_j$ in \eqref{eq:codes-clusters} is obtained by hard-thresholding, i.e., ${\z_j= \mathit{H}_{\gamma_c}(\omg_{k_j}\P_j\x)}$, where ${\mathit{H}_{\gamma_c}(\cdot)}$ represents a vector hard-thresholding operator that zeros out elements whose magnitudes are smaller than $\gamma_c$, and leaves other entries unchanged. Then the optimized class $\hat{k}_j$ for the $j$th patch is computed as follows~\cite{pwls-ultra2018}:}
\begin{equation}
\label{eq:clustering}
 \small{\hat{k}_j = \argmin_{1\leq k \leq K} || \omg_{k} \P_j \x - \mathit{H}_{\gamma_c}(\omg_{k}\P_j\x)||^2_2 + \gamma_c^2\|\mathit{H}_{\gamma_c}(\omg_{k}\P_j\x)\|_0. }
\end{equation} 
\DIFadd{We compute the cost values on the right hand side of \eqref{eq:clustering} for each $k = 1, \cdots, K$, and determine the $\hat{k}_j \in \{1, \cdots, K\}$ that gives the minimal cost value, i.e., patch $\P_j \x$ is grouped with the transform that provides the smallest value of the cost in \eqref{eq:clustering}. Then, the corresponding optimal sparse code is ${\hat{\z}_j = \mathit{H}_{\gamma_c}(\omg_{\hat{k}_j}\P_j\x)}$.}
\begin{algorithm}[!htp]  
	\caption{SPULTRA Algorithm}
	\label{alg: spultra-alg}
	\begin{algorithmic}[1]
		\Require~~\\
		initial image $\hat{\x}^{0}$; $\alpha = 1.999$ ; $\rho_0 = 1$; \\
		pre-computed $\D_\R $ according to \eqref{eq: D_R}\\
		number of outer iterations $N$, number of inner iterations $P$, and number of ordered-subsets $M$.	
		\Ensure reconstructed image $\hat{\x}^N$. 
		\For {$n=0,1,2,\cdots, N-1$}	
		\State \textbf{(1) Image Update}: Fix $\hat{\z}_j^{n}$ and $\hat{C}_k^n$; \\
		\textit{Initializations: 
		}\begin{enumerate}
			\item $\x^{(0)} =  \hat{\x}^{n}$,
			\item Determine $c_i(l^n_i)$ according to \eqref{eq:OptCuv},
			\item $\W^n = \diag\{c_i(l^n_i)\}$,
			\item $\D_{\A} \triangleq \diag\{\DIFadd{\A^T\W^n\A\mathbf{1}}\}$,			 				  		 
			\item \DIFadd{$\bm{d}_h(l^n) = [I_0e^{-f_i(l^n_i)}\dot{f_i}(l_i^n)(\frac{Y_i}{I_0e^{-l^n_i} + \sigma^2} - 1)]_{i = 1}^{N_d}$,	 
			}\item $\tilde{\y}^n = \A\x^{(0)} -{\W^n}^{-1}[\bm{d}_h(l^n)]^T$,
			\item $\ze^{(0)} = \g^{(0)} = M\A_M^T\W^n_M(\A_M\x^{(0)}-\tilde{\y}_M^n) $,
			\item $\bm{\eta}^{(0)} = \D_\A \x^{(0)} - \ze^{(0)}$, 
			\item compute $\nabla \R_2(\x)$ according to \eqref{eq:grad_r2}.
		\end{enumerate}
		%DIF > 	
		%DIF > 		$\qquad \qquad \W = \diag\{c_i(l^n_i)\}$,\\
		%DIF > 		$\D_{\A} \triangleq \diag\{|\A|^T|\W||\A|\mathbf{1}\}$,			 		\\			  		 
		%DIF > 		$\bm{d}_h(l^n) = [I_0e^{-l^n_i}(\frac{Y_i}{I_0e^{-l^n_i} + \sigma^2} - 1)]_{i = 1}^{N_d}$,\\		 
		%DIF > 		$\tilde{\y}^n = \A\x^{(n)} -\W^{-1}\bm{d}_h(l^n)^T$,\\
		%DIF > 		$\ze^{(0)} = \g^{(0)} = M\A_M^T\W(\A_M\x^{(n)}-\tilde{y}^n) $,\\
		%DIF > 		$\bm{\eta}^{(0)} = \D_\A \x^{(n)} - \ze^{(0)}$, \\
		%DIF > 		$\nabla \R_2(\x) = 2\beta\sum_{k=1}^{K} \sum_{j\in C_k} \tau_j \P_j^T \omg_{k}^T (\omg_k \P_j \x - \z_j)$;		
		\For {$p=0,1,2,3,\cdots,P-1$}	
		\For {$m=0,1,2,3,\cdots,M-1$}	
		\begin{equation*}\label{eq:rlalm}
		\begin{aligned}
		&t ~= ~pM + ~m;\\
		&\hspace{-0.1in}\left\{		
		\begin{aligned}
		\s^{(t+1)} &= \rho_t(\D_\A \x^{(t)} -\bm{\eta}^{(t)}) + (1-\rho_t)\g^{(t)} \\
		\x^{(t+1)} &= [\x^{(t)} - (\rho_t\D_\A+\D_\R)^{-1}(\s^{(t+1)} +\nabla \R_2(\x^{(t)}))]_\mathcal{C} \\
		\ze^{(t+1)}& \triangleq M\A_m^T\W^n_m(\A_m\x^{(t+1)}-\tilde{\y}_m^n)   \\
		\g^{(t+1)} &= \frac{\rho_t}{\rho_t+1}(\alpha \ze^{(t+1)} + (1-\alpha)\g^{(t)}) +  \frac{1}{\rho_t+1}\g^{(t)}\\
		\bm{\eta}^{(t+1)} &= \alpha(\D_{\A} \x^{(t+1)} -\ze^{(t+1)}) + (1-\alpha)\bm{\eta}^{(t)}	
		\end{aligned}
		\right.\\	
		&\text{Decrease $\rho_t$ according to \eqref{eq:rho}};
		\end{aligned}
		\end{equation*}  
		\EndFor	
		\EndFor				  	
		\State  $\hat{\x}^{n+1} = \x^{(t+1)}$;
		\State \textbf{(2) Sparse Coding and Clustering}: Fix $\hat{\x}^{n+1}$, compute class assignments $\hat{k}_j^{n+1}$ using \eqref{eq:clustering}, and sparse codes  $\hat{\z}_{j}^{n+1} =  H_{\DIFadd{\gamma_c}}(\omg_{\hat{k}_j^{n+1}} \P_j \hat{\x}^{n+1}),\   \forall \ j$. 
		\EndFor		
	\end{algorithmic} 
\end{algorithm}	

\textbf{Algorithm} \ref{alg: spultra-alg} illustrates the proposed optimization algorithm for Problem \eqref{eq:P0}.
\subsection{Computational Cost} \label{sec:computation analysis}
The SPULTRA algorithm has a similar structure in each iteration as the recent PWLS-ULTRA \cite{pwls-ultra2018}, except for several initializations in the image update step. Since forward and backward projections are used to compute $\D_\A$ and $\tilde{\y}^n$ during initialization, the image update step of SPULTRA is slightly slower than PWLS-ULTRA. In our experiments, we observed that the initializations took around $20 \%$ of the runtime in each outer iteration. However, in practice, especially for low doses, SPULTRA reconstructs images better than PWLS-ULTRA for a given number of outer iterations. Or alternatively, SPULTRA takes much fewer outer iterations (and runtime) to achieve the same image reconstruction quality as PWLS-ULTRA. These results are detailed in Sec. \ref{sec:experiments}.


